3D GameDev Arena: Benchmarking Coding Agents That Plan, Build, and Playtest extreme Long-Horizon Browser Games

Coding agents now resolve repository issues and generate compact playable games, but whether they can build a large 3D game from scratch remains open. Such games tightly couple mechanics, scenes, assets, and interaction logic, and their quality rests on player enjoyment, which existing benchmarks rarely assess. Thus, we introduce 3D GameDev Arena, a first extreme long-horizon benchmark of 108 from-scratch game-development tasks across 14 genres. Given only a text specification and UI/UX reference images, a fully automated plan--implement--test--repair pipeline builds each task into a self-contained browser game. Runs average $\sim$1,000 LLM calls ; the longest uses 14,407 calls, 2.13B tokens, and 608 assets. Evaluation spans (1) objective code-level functional acceptance against the game specification, (2) agent-based QA and playtesting of 3D presentation and playability, and (3) blind pairwise Bradley-Terry human preference in a public arena. The preliminary findings indicate that long-horizon 3D game development remains far from solved, and code-level correctness alone does not dictate player preference. The public arena is hosted online.

==> sections/long_horizon_addendum.tex <==
\subsection{Late-Stage Goal Alignment and Plan Adaptation}
\bizhe{this is needed, for analaysis of long-term strategy}
\label{sec:late-alignment}
% We supplement the website snapshot with a separate retrospective archive of 175 versions across 73 games, covering Astra/Codex, Sol/Codex, Kimi/Kimi Code, and GLM/ZCode. Its 53 structurally larger-task versions are grouped by requirement families and a bounded dependency graph, not human completion time or observed development duration. The two cohorts are not pooled. This addition reuses archived trajectory annotations and replay observations; it performs no new generation, gameplay execution, or annotation. Appendix~\ref{sec:retrospective-appendix} specifies the sources and aggregation.

% Two retrospective diagnostics address sustained development. \emph{Goal alignment} (LGR) measures whether observable actions support the then-valid requirements, including applicable procedural constraints. \emph{Initial-plan alignment} (LPA0) measures association with the first recoverable explicit pre-implementation plan. Each reports a conditional rate on adjudicable actions and a separate coverage measure; unknown evidence is not counted as aligned. Late-stage means the final operation-order quartile of the observed window, which may include authorized updates or publication work, rather than a predefined debugging phase. These diagnostics do not alter the functional or preference scores.

% \input{tables/retrospective-late}

% The larger-task samples show high late-stage conditional goal alignment, with different evidence coverage. They do not establish a universal late-stage collapse, nor does continued relevant work establish successful implementation. Sol's lower initial-plan association coexists with high goal alignment; the two valid game sets differ, so their rates cannot be subtracted to estimate a replanning frequency. The archive includes a concrete reason to separate the concepts: GLM's SP3D-135 coastal-defense task later received user authorization for an eight-wave mode beyond the original four-wave scope. Work on that extension need not violate the current goal. Authorized adaptation and unrequested deviation therefore require different interpretations; neither diagnostic directly measures internal memory.

% \subsection{Continuous Gameplay and 3D Integration}
% \label{sec:continuous-cases}
% Selected replay observations illustrate what remains invisible in aggregate development counts. Figure~\ref{fig:retrospective-cases} reconstructs three evidence sequences from the archived report, retaining their unexamined portions. These are illustrative cases across different tasks, not a comparative quality test.

% \begin{figure*}[tp]
% \centering
% \resizebox{\linewidth}{!}{\input{figures/retrospective-cases.tikz}}
% \caption{Schematic rendering of archived observations, not game screenshots or new experiments. Left: successive player actions connect combat, rewards, equipment, and another stage. Center: normal input produces climbing and landing progress in a 3D setting. Right: a rendered scene coexists with a stalled simulation. Arrows organize the reported sequence; they do not assert complete specification coverage or isolate the cause of a defect.}
% \label{fig:retrospective-cases}
% \end{figure*}

% For Kimi's SP3D-073 (\emph{Pok\'emon Quest}), normal play reached victory, returned to camp, equipped a reward stone with a corresponding attack-value change, and entered the next battle. This connects several game systems through player actions; cooking and the full campaign remain unverified. For Sol's SP3D-139 Paris rooftop scenario, normal Space input produced climbing and landing progress, providing a bounded example of input, movement, and spatial interaction. Complete assassination and escape were not established. Correcting the replay controller's initial loading wait is not evidence of the development agent repairing its own game.

% Astra's SP3D-233 (\emph{The Flame in the Flood}) supplies a contrasting reliability observation: a first-frame negative-delta-related \texttt{RangeError} recurred in fresh environments and after refresh while time and raft movement stalled despite a visible scene. This is a reference-protocol defect, not a demonstrated historical whole-game failure. Together, these cases motivate separate checks for visible presentation, runtime progression, and connected gameplay, without turning missing observations into failures.


==> tables/evaluation-metrics.tex <==
\begin{table*}[tp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Evaluation outputs, their scales, and how incomplete evidence is handled.}
\label{tab:evaluation-metrics}
\begin{tabularx}{\linewidth}{@{}p{0.24\linewidth}p{0.12\linewidth}Y@{}}
\toprule
Output & Scale & Unit and treatment of incomplete evidence \\
\midrule
Functional score & $[0,100]$ & Equal-weight valid criteria; each uses a fixed subitem denominator. Test errors and missing results leave coverage gaps. \\
Code coverage & $[0,1]$ & Valid / applicable criteria; configuration coverage uses summed counts across tasks. \\
3D presentation & $[0,100]$ & Expected win rate against fixed reference games, from blind side-by-side comparisons. \\
Playability & $[0,100]$ & Mean five-level rating of individual moments, covering control and flow. \\
Playtest coverage & $[0,1]$ & Observed / planned situations; unobserved situations are left out of the scores. \\
Human preference & $[0,100]$ & Expected win rate against other rated configurations; ties and both-bad are half-wins, skips excluded. \\
Generation success & $[0,1]$ & Playable artifacts / completed task--configuration runs; terminal failures are retained, infrastructure interruptions excluded. \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/retrospective-all.tex <==
\begin{table}[htbp]
\centering\small
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Goal retention (GR) and plan adherence (PA) in the last quarter of a run}, for all builds and for builds of large tasks.}
\label{tab:retrospective-all}
\begin{tabular}{lllrrr}
\toprule
Tasks & Configuration & Metric & Rate (\%) & Coverage (\%) & Bounds (\%) \\
\midrule
All & \texttt{gpt-6-astra} & GR & 100.00 & 91.85 & 91.85--100.00 \\
All & \texttt{gpt-6-astra} & PA & 98.79 & 78.99 & 78.08--99.09 \\
All & \texttt{gpt-6.1-sol} & GR & 99.71 & 89.15 & 88.94--99.79 \\
All & \texttt{gpt-6.1-sol} & PA & 96.64 & 83.47 & 81.14--97.67 \\
All & \texttt{kimi-k3} & GR & 94.09 & 82.50 & 77.50--95.00 \\
All & \texttt{kimi-k3} & PA & 97.62 & 86.94 & 85.28--98.33 \\
All & \texttt{glm-5.3} & GR & 100.00 & 93.75 & 93.75--100.00 \\
All & \texttt{glm-5.3} & PA & 100.00 & 43.75 & 43.75--100.00 \\
\midrule
Large & \texttt{gpt-6-astra} & GR & 100.00 & 93.48 & 93.48--100.00 \\
Large & \texttt{gpt-6-astra} & PA & 100.00 & 88.04 & 88.04--100.00 \\
Large & \texttt{gpt-6.1-sol} & GR & 100.00 & 92.19 & 92.19--100.00 \\
Large & \texttt{gpt-6.1-sol} & PA & 91.44 & 89.84 & 83.59--93.75 \\
Large & \texttt{kimi-k3} & GR & 96.23 & 72.12 & 69.23--97.12 \\
Large & \texttt{kimi-k3} & PA & 98.61 & 81.73 & 80.77--99.04 \\
Large & \texttt{glm-5.3} & GR & 100.00 & 100.00 & 100.00--100.00 \\
Large & \texttt{glm-5.3} & PA & 100.00 & 87.50 & 87.50--100.00 \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize Rate: share of aligned operations among those that could be judged. Coverage: share of operations that could be judged. Bounds: share of aligned operations if every unclear operation counted as deviating (lower) or as aligned (upper); they are not confidence intervals. \texttt{glm-5.3} has very few builds in this archive, so its values are indicative only.}
\end{table}


==> tables/retrospective-delegation.tex <==
\begin{table}[htbp]
\centering\small
\setlength{\tabcolsep}{4pt}
\caption{Root and descendant logical responses for SP3D-073.}
\label{tab:retrospective-delegation}
\begin{tabular}{lrrr}
\toprule
Configuration & Root & Descendants & Total \\
\midrule
Astra/Codex & 1,064 & 2,118 & 3,182 \\
Sol/Codex & 2,242 & 4,869 & 7,111 \\
Kimi/Kimi Code & 170 & 3,468 & 3,638 \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize Counts describe attributed observed windows, not tool calls, elapsed time, critical-path length, cost, or collaboration quality. Descendants can run in parallel; historical attribution and window completeness remain limitations.}
\end{table}


==> tables/retrospective-functional.tex <==
\begin{table*}[tp]
\centering\small
\setlength{\tabcolsep}{4pt}
\caption{Strict functional-evidence subset; conditional scores and full-cohort coverage.}
\label{tab:retrospective-functional}
\begin{tabular}{lrrr}
\toprule
Configuration & Observed/all & $F_{\mathrm{obs}}$ (\%) & Cohort coverage (\%) \\
\midrule
Astra/Codex & 7/69 & 72.30 & 6.00 \\
Sol/Codex & 6/59 & 77.18 & 6.38 \\
Kimi/Kimi Code & 6/45 & 74.91 & 6.88 \\
GLM/ZCode & 0/2 & -- & 0.00 \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize $F_{\mathrm{obs}}$ averages over versions with observed functional evidence. Coverage averages over every version of the configuration, including those with no functional evidence; it is not coverage of the scored subset. These retrospective atomic weights differ from the criterion-based Functional score in Section~\ref{sec:code-acceptance}.}
\end{table*}


==> tables/retrospective-late.tex <==
\begin{table*}[tp]
\centering\small
\setlength{\tabcolsep}{4pt}
\caption{Late-stage goal and initial-plan alignment on structurally larger tasks.}
\label{tab:retrospective-late}
\begin{tabular}{lrrrrrrr}
\toprule
Configuration & $N$ & LGR (\%) & Cov. (\%) & $n_G$ & LPA0 (\%) & Cov. (\%) & $n_P$ \\
\midrule
Astra/Codex & 23 & 100.00 & 93.48 & 23 & 100.00 & 88.04 & 22 \\
Sol/Codex & 16 & 100.00 & 92.19 & 16 & 91.44 & 89.84 & 15 \\
Kimi/Kimi Code & 13 & 96.23 & 72.12 & 12 & 98.61 & 81.73 & 12 \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize $N$: all versions in this structural group; $n_G,n_P$: games with defined conditional rates. Rates are game-equal means on adjudicable actions in operation quartile 4; coverage retains unknown evidence. A value of 100\% does not certify unsampled actions. The two metrics can have different valid game sets. GLM ($N=1$) is reported in Appendix~\ref{sec:retrospective-appendix}.}
\end{table*}


==> tables/task-specification.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\linewidth}{@{}p{0.32\linewidth}Y@{}}
\toprule
Common specification part & Role in the task \\
\midrule
Role and Objective & Sets the development objective, required experience, and bounded scope. \\
Game Overview and Player Experience & Describes the intended experience and, where supplied, visual references. \\
Project Setup and Deliverables & States the task's source, build, runtime, and delivery requirements. \\
Complete Game Design & Connects controls, mechanics, state and resources to a player-activity loop and its outcomes. \\
Acceptance Criteria & States observable conditions for checking the requested behavior and delivery. \\
\bottomrule
\end{tabularx}
\caption{Common semantic structure of the game-development task specifications. Each task instantiates these five parts through its intended experience, mechanics, implementation requirements, and observable acceptance conditions.}
\label{tab:task-specification}
\end{table}


==> tables/web-calls.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\caption{Additional call summaries. Parentheses give non-partial sample sizes; $N$ is the number of published results.}
\label{tab:web-calls}
\begin{tabular}{lrrrr}
\toprule
ID & $N$ & Model responses & Execution calls & Unclassified debug \\
\midrule
01 & 1 & 111.0 (1) & 123.0 (1) & 0.0 (1) \\
02 & 1 & 264.0 (1) & 391.0 (1) & 0.0 (1) \\
03 & 10 & 2,266.0 (10) & 1,699.0 (10) & 30.5 (10) \\
04 & 25 & 1,164.0 (22) & 822.0 (22) & 19.5 (22) \\
05 & 1 & 1,313.0 (1) & 996.0 (1) & 10.0 (1) \\
06 & 18 & 1,402.0 (17) & 1,022.0 (17) & 18.0 (17) \\
07 & 13 & 828.0 (8) & 1,118.0 (8) & 3.0 (12) \\
08 & 1 & 1,703.0 (1) & 1,854.0 (1) & 4.0 (1) \\
11 & 5 & 454.5 (4) & 532.5 (4) & 23.0 (4) \\
12 & 2 & 681.5 (2) & 765.0 (2) & 43.0 (2) \\
13 & 4 & 498.0 (4) & 955.5 (4) & 0.5 (4) \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize Entries are medians, or individual values for singleton observations. All included call records are approximate. Unclassified debug counts are separate from the visual and headless categories. Quartiles and missing-value counts for every field are supplied in the analysis package.}
\end{table}


==> tables/web-configurations.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Configuration identities and published-result coverage in the website snapshot. Empty effort fields are reported as unspecified.}
\label{tab:web-configurations}
\begin{tabular}{llllr}
\toprule
ID & Model & Harness & Effort & $N$ \\
\midrule
01 & Claude Opus 5 & Claude Code & -- & 1 \\
02 & Claude Sonnet 5 & Claude Code & -- & 1 \\
03 & GPT 5.6 Sol & Codex & ultra & 10 \\
04 & GPT 6 Astra & Codex & ultra & 25 \\
05 & GPT 6 Sol & Codex & ultra & 1 \\
06 & GPT 6.1 Sol & Codex & ultra & 18 \\
07 & Kimi K3 & Kimi Code & max & 13 \\
08 & Qwen 3.8 & OpenHands & max & 1 \\
09 & DeepSeek V4 Pro & OpenHands & -- & 0 \\
10 & DeepSeek V4 Pro & Pi & -- & 0 \\
11 & Qwen 3.8 & Pi & max & 5 \\
12 & GLM 5.3 & ZCode & max & 2 \\
13 & Grok 4.7 & GrokBuild & xhigh & 4 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/web-paired.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Descriptive comparison on shared prompts: GPT 6 Astra and GPT 6.1 Sol, both with Codex. Each row uses its own complete, non-partial pairs.}
\label{tab:web-paired}
\begin{tabular}{lrrrr}
\toprule
Metric & $n$ & Astra & 6.1 Sol & Paired $\Delta$ \\
\midrule
All tool calls & 14 & 1,016.50 & 1,321.00 & +255.00 \\
Visual debug calls & 15 & 49.00 & 59.00 & +19.00 \\
Headless debug calls & 15 & 4.00 & 5.00 & +1.00 \\
Reported time (min) & 14 & 153.09 & 219.30 & +54.89 \\
Reported cost (RMB) & 14 & 1,352.27 & 230.99 & -1,005.36 \\
Output tokens (M) & 14 & 0.54 & 0.67 & +0.24 \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize Columns report medians. $\Delta$ is the median per-task difference (6.1 Sol minus Astra), not the difference of marginal medians. Calls are approximate; output tokens are exact-audit records. Reported time and cost have no per-field precision flag. No significance or causal claim is made.}
\end{table}


==> tables/web-resources.tex <==
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Reported resources and website scores, shown side by side without an efficiency ranking. Parentheses give the number of available resource observations.}
\label{tab:web-resources}
\begin{tabular}{lrrrr}
\toprule
ID & Time, min & Cost, RMB & Preference [95\% CI] & Code \\
\midrule
01 & 38.0 (1) & 471.0 (1) & 99.8 [99.5, 100.0] & -- \\
02 & 148.2 (1) & 195.0 (1) & 90.0 [89.7, 90.2] & -- \\
03 & 279.8 (10) & 1,075.7 (10) & 47.8 [40.3, 55.4] & -- \\
04 & 159.0 (24) & 1,352.3 (24) & 70.5 [63.6, 77.4] & 58.39 \\
05 & 1,135.3 (1) & 346.3 (1) & 62.7 [44.5, 80.8] & -- \\
06 & 229.7 (17) & 243.0 (17) & 62.9 [56.1, 69.7] & 49.24 \\
07 & 679.5 (13) & 631.3 (3) & 28.4 [21.6, 35.1] & 50.28 \\
08 & 1,280.1 (1) & -- & 13.0 [6.5, 19.4] & -- \\
11 & 447.8 (5) & 297.2 (4) & 19.8 [10.7, 28.8] & -- \\
12 & 185.2 (2) & 163.3 (2) & 25.9 [12.1, 39.8] & 21.81 \\
13 & 179.3 (4) & 85.8 (1) & 29.3 [17.5, 41.1] & -- \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize Resource entries are medians; singleton entries are individual values. Preference intervals are copied from the site, not recomputed. Code scores are page-provided configuration aggregates with no scored-task mapping. The scoring cohorts need not match the resource cohorts. IDs refer to Table~\ref{tab:web-configurations}.}
\end{table}


==> tables/web-tokens.tex <==
\begin{table*}[tp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Token medians in millions, using only fields marked exact by the website. Parentheses give valid sample sizes; missing records are not zeros.}
\label{tab:web-tokens}
\begin{tabular}{lrrrr}
\toprule
ID & $N$ & Uncached input & Cached input & Output \\
\midrule
01 & 1 & 7.8 (1) & 26.0 (1) & 0.1 (1) \\
02 & 1 & 4.9 (1) & 37.3 (1) & 0.8 (1) \\
03 & 10 & 6.8 (10) & 259.0 (10) & 1.0 (10) \\
04 & 25 & 3.3 (22) & 127.2 (22) & 0.5 (22) \\
05 & 1 & 5.7 (1) & 158.3 (1) & 0.5 (1) \\
06 & 18 & 4.4 (17) & 162.3 (17) & 0.7 (17) \\
07 & 13 & -- & -- & -- \\
08 & 1 & 4.9 (1) & 152.0 (1) & 2.2 (1) \\
11 & 5 & 2.3 (1) & 196.7 (1) & 0.7 (1) \\
12 & 2 & 7.2 (2) & 106.0 (2) & 0.7 (2) \\
13 & 4 & 1.9 (1) & 39.0 (1) & 0.3 (1) \\
\bottomrule
\end{tabular}
\par\smallskip{\footnotesize Cache writes are included in uncached input by the website. Partial and unavailable native usage records are excluded from these medians and retained in the analysis package.}
\end{table*}

